Private Text Generation by Seeding Large Language Model Prompts

We explore how private synthetic text can be generated by suitably prompting a large language model (LLM). This addresses a challenge for organizations like hospitals, which hold sensitive text data like patient medical records, and wish to share it in order to train machine learning models for medical tasks, while preserving patient privacy. Methods that rely on training or finetuning a model may be out of reach, either due to API limits of third-party LLMs, or due to ethical and legal prohibitions on sharing the private data with the LLM itself. We propose Differentially Private Keyphrase Prompt Seeding (DP-KPS), a method that generates a private synthetic text corpus from a sensitive input corpus, by accessing an LLM only through privatized prompts. It is based on seeding the prompts with private samples from a distribution over phrase embeddings, thus capturing the input corpus while achieving requisite output diversity and maintaining differential privacy. We evaluate DP-KPS on downstream ML text classification tasks, and show that the corpora it generates preserve much of the predictive power of the original ones. Our findings offer hope that institutions can reap ML insights by privately sharing data with simple prompts and little compute.

==> discussion.tex <==
\section{Discussion}
\begin{itemize}
\item We studied text data only, but real data is accompanied by numeric data, time-series data, images, etc.
\end{itemize}

==> raw_tables.tex <==
\small{
\begin{table}
{
% \renewcommand{\arraystretch}{2}
\begin{centering}
\begin{tabular}{c c c c c}
\toprule
Method &  eps voc & eps kde & Accuracy \\
\midrule
\rule{0pt}{3ex}
{} &   1 & 5 & 72.8\% \\
{}  & 1 & 10 & 77\% \\
{} &  1 & infinity & 86.6\% \\
\cline{2-4}
\rule{0pt}{3ex}
{} &  5 & 5 & 77.1\% \\
Baseline  & 5 & 10 & 81.2\% \\
{} &  5 & infinity & 82.4\% \\
\cline{2-4}
\rule{0pt}{3ex}
{} &  infinity & 5 & 76.5\% \\
  & infinity & 10 & 75.1\% \\
{} & infinity & infinity & 83.4\% \\
\midrule
\rule{0pt}{3ex}
{} &   1 & 5 & 30.0\% \\
{}  & 1 & 10 &  29.13\%\\
{} &  1 & infinity & 26.12\% \\
\cline{2-4}
\rule{0pt}{3ex}
{} &  5 & 5 &  24.76\%\\
Independent Baseline  & 5 & 10 &  26.38\%\\
{} &  5 & infinity & 29.88\% \\
\cline{2-4}
\rule{0pt}{3ex}
{} &  infinity & 5 & 22.27\% \\
  & infinity & 10 &  25.22\%\\
{} & infinity & infinity & 25.69\% \\
\midrule
\rule{0pt}{3ex}
{} &   1 & 5 & 78.25\% \\
{}  & 1 & 10 & 81.11\% \\
{} &  1 & infinity & 79.02\% \\
\cline{2-4}
\rule{0pt}{3ex}
{} &  5 & 5 & 80.97\% \\
ZeroBW  & 5 & 10 & 77.50\% \\
{} &  5 & infinity & 78.90\% \\
\cline{2-4}
\rule{0pt}{3ex}
{} &  infinity & 5 & 73.96\% \\
  & infinity & 10 & 78.36\% \\
{} & infinity & infinity & 77.25\% \\
\bottomrule
\end{tabular}
\caption{Performance of models trained on private-synthetic text on DBPedia-14 classification.} \label{tbl:datasets}
\end{centering}}
\end{table}
}


\small{
\begin{table}
{
% \renewcommand{\arraystretch}{2}
\begin{centering}
\begin{tabular}{c c c c}
\toprule
eps voc & eps kde & Accuracy \\
\midrule
\rule{0pt}{3ex}
   1 & 0.01 & 57.2\% \\
 1 & 5 & 58.7\% \\
 1 & 10 & 55\% \\
 1 & 5000 & 59.6\% \\
\hline
\rule{0pt}{3ex}
  5 & 0.01 & 53.5\% \\
 5 & 5 & 58.4\% \\
 5 & 10 & 60.3\% \\
 5 & 5000 & 64.4\% \\
\hline
\rule{0pt}{3ex}
  infinity & 0.01 & 48.6\% \\
 infinity & 5 & 68.6\% \\
 infinity & 10 & 68.5\% \\
 infinity & 5000 & 60.7\% \\
\bottomrule
\end{tabular}
\caption{ Private synthetic text generated using the Independent baseline method. Performance of models trained on private-synthetic text on MIMIC heart failure classification.} \label{tbl:mimic_results}
\end{centering}}
\end{table}
}





\small{
\begin{table}
{
% \renewcommand{\arraystretch}{2}
\begin{centering}
\begin{tabular}{c c c c c}
\toprule
Method &  eps voc & eps kde & Accuracy \\
\midrule
\rule{0pt}{3ex}
{} &   1 & 5 & 77.9\% \\
{}  & 1 & 10 & 82.4\% \\
{} &  1 & infinity & 87.5\% \\
\cline{2-4}
\rule{0pt}{3ex}
{} &  5 & 5 & 80.4\% \\
Baseline  & 5 & 10 & 85.1\% \\
{} &  5 & infinity & 85.9\% \\
\cline{2-4}
\rule{0pt}{3ex}
{} &  infinity & 5 & 80.9\% \\
  & infinity & 10 & 82.3\% \\
{} & infinity & infinity & 85.5\% \\
\midrule
\rule{0pt}{3ex}
{} &   1 & 5 & 30.24\% \\
{}  & 1 & 10 &  29.04\%\\
{} &  1 & infinity &  30.98\%\\
\cline{2-4}
\rule{0pt}{3ex}
{} &  5 & 5 &  24.09\%\\
Independent Baseline  & 5 & 10 &  24.25\%\\
{} &  5 & infinity &  \\
\cline{2-4}
\rule{0pt}{3ex}
{} &  infinity & 5 & 24.13\% \\
  & infinity & 10 &  26.13\%\\
{} & infinity & infinity &  29.34\%\\
\midrule
\rule{0pt}{3ex}
{} &   1 & 5 & 82.16\% \\
{}  & 1 & 10 & 83.83\% \\
{} &  1 & infinity & 85.73\% \\
\cline{2-4}
\rule{0pt}{3ex}
{} &  5 & 5 &  86.05\%\\
ZeroBW  & 5 & 10 &  82.39\%\\
{} &  5 & infinity & 83.97\% \\
\cline{2-4}
\rule{0pt}{3ex}
{} &  infinity & 5 & 80.26\% \\
  & infinity & 10 & 84.28\% \\
{} & infinity & infinity & 85.64\% \\
\bottomrule
\end{tabular}
\caption{Performance of classification models trained on private-synthetic text with domain adaptation using DeepCoral~\cite{sun2016deep} on DBPedia-14 classification.} \label{tbl:datasets}
\end{centering}}
\end{table}
}


\small{
\begin{table}
{
% \renewcommand{\arraystretch}{2}
\begin{centering}
\begin{tabular}{c c c c}
\toprule
eps voc & eps kde & Accuracy \\
\midrule
\rule{0pt}{3ex}
   1 & 0.01 & 50.7\% \\
 1 & 5 & 71.6\% \\
 1 & 10 & 72.2\% \\
 1 & 5000 & 70\% \\
\hline
\rule{0pt}{3ex}
  5 & 0.01 & 56\% \\
 5 & 5 & 71.7\% \\
 5 & 10 & 72.2\% \\
 5 & 5000 & 69.7\% \\
\hline
\rule{0pt}{3ex}
  infinity & 0.01 & 55.7\% \\
 infinity & 5 & 71.1\% \\
 infinity & 10 & 71\% \\
 infinity & 5000 & 70.8\% \\
\bottomrule
\end{tabular}
\caption{ Private synthetic text generated using the Independent baseline method. Performance of classification models trained on private-synthetic text using DeepCoral~\cite{sun2016deep} on MIMIC heart failure classification.} \label{tbl:mimic_results_da}
\end{centering}}
\end{table}
}
